Crowd simulation incorporating a route choice model and similarity evaluation using real large-scale data

Modeling and simulation approaches that express crowd movement with mathematical models are widely and actively studied to understand crowd movement and resolve crowd accidents. Existing literature on crowd modeling focuses on only the decision-making of walking behavior. However, the decision-making of route choice, which is a higher-level decision, should also be modeled for constructing more practical simulations. Furthermore, the reproducibility evaluation of the crowd simulation incorporating the route choice model using real data is insufficient. Therefore, we generalize and propose a crowd simulation framework that includes actual crowd movement measurements, route choice model estimation, and crowd simulator construction. We use the Discrete choice model as the route choice model and the Social force model as the walking model. In experiments, we measure crowd movements during an evacuation drill in a theater and a firework event where tens of thousands of people moved and prove that the crowd simulation incorporating the route choice model can reproduce the real large-scale crowd movement more accurately.

==> tab/literature.tex <==
\begin{tabular}{lll}
\hline
                                           & Route choice model is estimated using real data & Crowd simulation is evaluated using real data \\ \hline
{[}Liu+, 2012{]}                           & $\times$   &  $\times$  \\
{[}Lovreglio+, 2016{]}                     & $\bigtriangleup$  &  $\times$   \\
{[}Haghani+, 2017{]}, {[}Haghani+, 2019{]} & $\bigcirc$  &  $\bigtriangleup$  \\
{[}Gao+, 2019{]}                           & $\times$   & $\bigcirc$   \\
{[}Yang+, 2020{]}                          & $\times$   & $\times$    \\
{[}Lu+, 2021{]}                            & $\bigtriangleup$  & $\times$ \\
Ours                                       &  $\bigcirc$  &  $\bigcirc$   \\ \hline
\end{tabular}


==> tab/shinkoku_model_parameters.tex <==
\centering
\scalebox{1.0}[1.0]{
\begin{tabular}{|l|l|}
\hline
parameters   & estimate  \\ \hline \hline
$\beta_{\rm DIST}$ & -1.33  \\ \hline
$\beta_{\rm CH}$  &  1.13 \\ \hline
$\beta_{\rm NF}$  & 0.202 \\ \hline
$\beta_{\rm NB}$  & -0.105 \\ \hline
ASC$_{Route 2}$ & 2.33 \\ \hline \hline
Accuracy [\%] & 82.2 \\ \hline
\end{tabular}
}
